T-SCI: A Two-Stage Conformal Inference Algorithm with Guaranteed Coverage for Cox-MLP

It is challenging to deal with censored data, where we only have access to the incomplete information of survival time instead of its exact value. Fortunately, under linear predictor assumption, people can obtain guaranteed coverage for the confidence band of survival time using methods like Cox Regression. However, when relaxing the linear assumption with neural networks (e.g., Cox-MLP (Katzman et al., 2018; Kvamme et al., 2019)), we lose the guaranteed coverage. To recover the guaranteed coverage without linear assumption, we propose two algorithms based on conformal inference. In the first algorithm WCCI, we revisit weighted conformal inference and introduce a new non-conformity score based on partial likelihood. We then propose a two-stage algorithm T-SCI, where we run WCCI in the first stage and apply quantile conformal inference to calibrate the results in the second stage. Theoretical analysis shows that T-SCI returns guaranteed coverage under milder assumptions than WCCI. We conduct extensive experiments on synthetic data and real data using different methods, which validate our analysis.

==> text/garbage.tex <==
% Firstly, we focus on samples ${n+1}$ generated from $\tilde{Q}_X(x)$ where we assume that $\tilde{Q}_X<<\tilde{P}_X$,that is $\tilde{Q}_X$ as a probability measure is absolutely continuous with respect to measure $\tilde{P}_X$. Therefore, the Radon-Nikodym derivative $\frac{\mathrm{d}\tilde{Q}_X}{\mathrm{d}\tilde{P}_X}$ exists and we denote it as $\hat{w}$, i.e. $\mathrm{d}\tilde{Q}_X(x) = \hat{w}(x) \mathrm{d} \tilde{P}_X(x)$.
% We would prove that the probability that $\tilde{T}^\prime$ falls in the derived confidence interval $\hat{C}^1_n(X^\prime)$ is larger than $1-\alpha$, where $\alpha$ is the given significance level.
% The intuition is that, since the derived $\hat{C}^1_n(X^\prime)$ is derived based on the estimated weight $\hat{w}(x)$, the sample $\tilde{T}^\prime$ is then guaranteed to fall in the confidence interval with probability at least $1-\alpha$.

% \begin{equation}
% \begin{split}
% & \mathbb{P}\left(\tilde T^\prime \in \hat{C}^1_n(X^\prime) | \mathcal{Z}_{tr}\right) \\
% =& \mathbb{P}\left(T_l(X^\prime) \leq \tilde T^\prime \leq T_r(X^\prime) | \mathcal{Z}_{tr}\right) \\
% =& \mathbb{P}\left( g(x_i) - \log\sum_{k\in R(T_l)} g(x_k) \leq  g(x_i) - \log\sum_{k\in R(T^\prime)} g(x_k) \leq g(x_i) - \log\sum_{k\in R(T_r)} g(x_k) | \mathcal{Z}_{tr}\right) \\
% =& \mathbb{P} \left(\tilde V(\tilde{X}^\prime, \tilde T^\prime) \in \operatorname{Quantile} \left(1-\alpha; \sum_{i=1}^n \hat{p}_i \delta_{v_i}+\hat{p}_\infty \delta_{\infty}\right) | \mathcal{Z}_{tr}\right) \\
% \overset{(i)}{=}& \mathbb{P} \left(\tilde V(\tilde{X}^\prime, \tilde T^\prime) \in \operatorname{Quantile} \left(1-\alpha; \sum_{i=1}^n \hat{p}_i \delta_{v_i}+\hat{p}_\infty \delta_{V(\tilde{X}^\prime, \tilde T^\prime)}\right) | \mathcal{Z}_{tr}\right) \\
% =& \mathbb{E}_\mathcal{E} \mathbb{P} \left(\tilde V(\tilde{X}^\prime, \tilde T^\prime) \in \operatorname{Quantile} \left(1-\alpha; \sum_{i=1}^n \hat{p}_i \delta_{v_i}+\hat{p}_\infty \delta_{V(\tilde{X}^\prime, \tilde T^\prime)}\right) | \mathcal{Z}_{tr}, \ \mathcal{E} (\tilde V) \right) \\
% \overset{(ii)}{\geq}& 1-\alpha
% \end{split} 
% \end{equation} 

% The Equation (i) is due to Lemma~\ref{lem:equiv}, and the Equation (ii) is due to Lemma~\ref{lem:vprob}.

From \citet{lei2020conformal} (Page 33), we have for a fixed $\epsilon$,
\begin{equation*}
    \begin{split}
\mathbb{P}(Y \in \hat{C}(X) | X) \geq 1 - \alpha - b_2 (\epsilon + H(X)) - I(H(X) > \epsilon) - \mathbb{P}(\eta < -\epsilon)
    \end{split}
\end{equation*}

By taking expectations on $X$, we have
\begin{equation*}
    \begin{split}
\mathbb{P}(Y \in \hat{C}(X) ) \geq 1 - \alpha - b_2 (\epsilon + \mathbb{E} H(X)) - \mathbb{P}(H(X) > \epsilon) - \mathbb{P}(\eta < -\epsilon)
    \end{split}
\end{equation*}

\jiaye{where to use $2\epsilon < r$}

Since $H(X) \leq B$ almost surely, by taking $\epsilon=B+\gamma$, we have 
\begin{equation*}
\mathbb{P}(Y \in \hat{C}(X) ) \geq 1 - \alpha - b_2 (2B + \gamma)  - \mathbb{P}(\eta < -(B+\gamma))
\end{equation*}

On the other hand, as $n \to \infty$
\begin{equation*}
\begin{split}
&\mathbb{P}(\eta < -(B+\gamma))   \\
\leq& \frac{16}{\epsilon^2 b_1} \mathbb{E}[\hat{w}(X) H(X)] \\
\leq& \frac{16B}{\epsilon^2 b_1}
\end{split}
\end{equation*}

Therefore, 
\begin{equation*}
\mathbb{P}(Y \in \hat{C}(X) ) \geq 1 - \alpha - b_2 (2B + \gamma)  - \frac{16B}{(B+\epsilon)^2 b_1}
\end{equation*}

\subsection{Proof of Theorem~\ref{thm: upperbound}}
Let $(X,Y)$ be generated from $\mathcal{P}_{XY}$, then 
\begin{equation*}
\begin{split}
    & \mathbb{P}(Y \in \hat{C}^2(X) | X ) \\
    =& \mathbb{P}(\min \{ \hat{q}(X) \})
\end{split}
\end{equation*}


==> text/temp.tex <==

\newpage
% The following is in the appendix.



% \textbf{Datasets and Environment.}
% We conduct extensive experiments to test the efficiency of the algorithm. 
% We use one synthetic dataset {RRNLNPH} (from \citet{kvamme2019time}) and two real-world datasets, METABRIC and SUPPORT (See supplementary materials for more details). 
% % We defer the characteristics of these datasets in .
% % We provide some characteristics of these datasets in \autoref{tab:datasets}. 
% % We conduct all experiments on Ubuntu server with AMD 3990X.
% % All experiments are run on Ubuntu server with AMD 3990X. All codes are programmed in Python. 
% % \begin{table}
% %     \centering
% %     \begin{tabular}{ccccc}
% %     \hline 
% %     Datasets     & \# data &  censored  & \# vars. & duration  \\
% %     \hline\hline 
% %       METABRIC  & 1904 & 42.1\% & 9 & [0.0,355.20]\\
% %       SUPPORT & 8873 & 32.0\% & 14 & [3.0,2029.0\\
% %       RR\_NL\_ NPH & 10000 & 33.03 \% & 3 & [0.0, 30.0]\\
% %       \hline 
% %     \end{tabular}
% %     \caption{Characteristics of Datasets}
% %     \label{tab:datasets}
% % \end{table}
% % \textbf{Procedure.} 
% For each datasets, we test several algorithms along with our proposed algorithms.
% In each run, 80\% data are randomly sampled as the training data and the two halves of the rest are randomly split as calibration data and test data.
% We run the experiments 100 times for each algorithm. 
% Moreover, we collect the results under different $\alpha$s. 


% \textbf{Algorithms.}
% We choose the linear Cox regression (labeled as Cox Reg.) as the baseline.
% Besides, we conduct CoxPH (i.e., DeepSurv \citet{katzman2018deepsurv}) and CoxCC \citep{kvamme2019time} (both belong to Cox-MLP) using $S(t)$ to return confidence band although they do not contain a theoretical guarantee.
% We also choose a kernel-based non-Cox methods, \citep{chen2020deep}, labeled as Kernel.
% We emphasize that Kernel is a different approach since our method is Cox-based. 
% % And the experimental results show that Kernel and T-SCI both reach a satisfying coverage.

% We integrate our proposed algorithms WCCI and T-SCI with CoxPH and CoxCC, labeled as CoxPH/CoxCC + WCCI/T-SCI.
% Besides, note that weight appears in WCCI and T-SCI.
% To ensure that the weight is helpful, we test the \emph{unweighted version} of WCCI and T-SCI where we set all weights to 1 in WCCI and T-SCI .


% As neural network is used as the nonlinear predictor in CoxPH and CoxCC, Cox Regression is chose to be the baseline linear predictor. Recently, \citet{chen2020deep} proposed a neural network based kernel survival analysis method. His algorithm is the state-of-the-art. We run his codes on the same datasets and compare with our algorithms. Results show that our algorithms are competitive.

% The experiment results where $\alpha=0.95$ are listed in \autoref{tab:rr_res}, \autoref{tab:s_res} and \autoref{tab:m_res}.



 
% Our main results provide guranteed coverage on survival time. Thus, empirical coverage of predicted survival time is used as an important performance index. 
% Empirical coverage is calculated as the fraction of testing points whose true survival time is no greater than predicted time. 
% Larger empirical coverage does not imply better performance as a trivial prediction is infinity and it will obtain coverage of 100\% in all cases. 
% Given confidence level $\alpha$, a perfect predictor is expected to return prediction results that have empirical coverage that equals to $\alpha$.
% As perfect predictor cannot be obtained in practice, we expect a better algorithm to have coverage that approximates $\alpha$ better. 
% Along with empirical coverage, we evaluate our algorithm by examine the length of predicted interval, which is the upper bound of predicted interval minus its lower counterpart. 
% More compact interval implies more "accurate" prediction. In our experiments, we evaluate the performance of different algorithms on both empirical coverage and prediction interval length. 


% \subsection{Analysis}
% We summarize the whole experimental results on dataset RRNLNPH in Table~\ref{tab:rr_res}. We defer the results on SUPPORT and METABRIC in the supplementary materials due to space limitations.

% \textbf{Coverage and Interval Length.}
% Figure~\ref{fig: coveragelength} shows the empirical coverage and the interval length of the confidence band returned by algorithms under difference confidence level $\alpha$.
% Ideally, the confidence band should have large coverage with small interval length.
% Notice that WCCI and T-SCI based algorithms outperform its original versions (usually underestimate), showing the effectiveness of the proposed algorithms.
% Furthermore, T-SCI is shown to be more conservative than WCCI, where T-SCI have larger coverage and interval length.
% We further remark that T-SCI returns guaranteed coverage under different confidence levels.

% Figure~\ref{fig: coveragelength}\zeren{??} illustrates that T-SCI returns large coverage with competitive interval length.



%\zeren{关于图4：\\首先是单纯的coxph coxcc比较差，加上了WCCI,T-SCI后效果较好，这说明了我们算法的有效性，
% 其次WCCI based算法比T-SCI based算法预测的coverage更小，不够准，相对于T-SCI激进（这会不会存在什么现实问题、风险？）；
% 再者，unweighted版本比weighted版本预测更激进，同时方差也较大，说明了WCI是不是有什么问题，是否和数据有关；(后面已经写了关于weight)
% 右图显示出unweighted的区间长度较小，这于他们的coverage更小是相符合的，但是方差却大很多，weighted的在不同的alpha的方差几乎一致；同样的，T-SCI比WCCI保守。}


% \textbf{The rationality of weight $w(x)$.}
% % \zeren{The effectiveness of WCI?}
% We show the comparison between weighted and unweighted versions in Figure~\ref{fig: weight}. 
% For WCCI algorithms, the weighted version has coverage closer to $(1-\alpha)$.
% % \zeren{??}
% And for T-SCI algorithms, the weighted version has a lower variance. 
% These results show that weighted versions outperform the unweighted versions, which validates the role of weight $w(x)$. 
% % These results show that weighted versions outperform the unweighted versions, which validates the covariate shift phenomenon. 
% % \zeren{too weak}


% \textbf{The difficulty in censoring.}
% Figure~\ref{fig: censor} shows the algorithms' performance on censored and uncensored data, respectively.
% All the algorithms performs larger coverage and less variance on the uncensored data, meaning that censored data is indeed more difficult to deal with than uncensored data.

% \textbf{Analysis of Table~\ref{tab:rr_res}.}
% We show RRNLNPH results in Table~\ref{tab:rr_res}, and results of SUPPORT and METABRIC performs similarly.
% Firstly, notice that WCCI always does not reach the expected coverage mainly due to the inaccurate estimation on the weight, while T-SCI reaches it due to a milder requirements in Theorem~\ref{thm: double robust} (double robustness).
% Secondly, notice that Cox Reg., CoxPH, CoxCC all fail to return the reasonable coverage, and they also lack theoretical guarantee.
% % Thirdly, we remark that T-SCI based methods show a large coverage on the censored data.
% Thirdly, unweighted versions all suffer from poor performances on censored data due to the lack of weight, showing that weight is important in dealing with covariate shift.
% Finally, we emphasize that although Kernel methods perform better in terms of coverage, it suffers from a large interval length and large variance. As a comparison, WCCI and T-SCI often perform more stably.

% \zeren{\\1. CoxPH, CoxCC包括加上WCCI,T-SCI效果都差不多；
% \\2. Cox Reg. CoxPH,CoxCC差不多；
% \\3. 算法1常常达不到coverage gurantee；
% \\4. unweighted 虽然总体表现好，但是在censor data上预测很不准，在所有数据集上预测得区间长度很大，coverage和length的方差都很大，在SUPPORT上尤其明显，WCCI的unweighted在SUPPORT上没达到level,差距很大，在censor上的结果很差，在metabric上的censor的coverage也不好；
% \\5. kernel效果较好，但是预测得区间长度很大，并且方差非常大，甚至metabric上在censor上的coverage更大；T-SCI在所有数据集上表现都比较稳定，并且都能保证coverage，censor uncensor页比较稳定
% }















\begin{figure*}
    \centering
    \includegraphics[width=13cm]{fig/shift_2.pdf}
    \caption{\textcolor{blue}{one of two should be removed}}
    \label{fig:my_label}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=15cm]{fig/diff_methods_rr.pdf}
    \caption{rr nl nph}
    \label{fig:my_label}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=15cm]{fig/diff_methods_support.pdf}
    \caption{support}
    \label{fig:my_label}
\end{figure*}


% Method Mean Std.
% Cox Reg 0.832 0.008
% Cox cc 0.829 0.008
% Cox PH  0.830 0.008
% WCCI+Cox PH 0.912 
% TSCI+COXPH 0.974
% CENSOR 0.854 0.947
% Non Censor 0.949 0.994
% WCCI+Cox CC 0.919
% TSCI+COX CC 0.974
% CENSOR 0.862 0.946
% Non Censor 0.955 0.995

% unweighted cox ph 0.907 0.950
% censor 0.830 0.875
% uncensor 0.949 0.991

% kernel 0.951 0.024

% metabric

% Method Mean Std.
% Cox Reg 0996 0.003
% Cox cc 0.996 0.003
% Cox PH  0.993 0.004
% WCCI+Cox PH 0.977
% TSCI+COXPH 0.986
% CENSOR 0.948 0.970
% Non Censor 0.985 0.989
% WCCI+Cox CC 0.973
% TSCI+COX CC 0.986
% CENSOR 0.942 0.971
% Non Censor 0.980 0.990

% unweighted cox ph 0.946 0.958
% censor 0.910 0.932
% uncensor 0.972 0.977

% kernel 0.981 0.025

% support

% Method Mean Std.
% Cox Reg 0.999 0.001
% Cox cc 0.999 0.001
% Cox PH  0.998 0.001

% WCCI+Cox PH 0.982
% TSCI+COX PH 0.993
% CENSOR 0.838 0.923
% Non Censor 0.984 0.993
% WCCI+Cox CC 0.980
% TSCI+COXCC 0.992
% CENSOR 0.829 0.916
% Non Censor 0.983 0.992
% unweighted cox ph 0.825 0.944
% censor 0.543 0.831
% uncensor 0.957 0.996

% kernel 0.95 0.024






\begin{table*}
    \centering
   \begin{tabular}{ccccccccc}
    \hline 
        Method & \multicolumn{2}{c}{Total} & \multicolumn{2}{c}{Censored} & \multicolumn{2}{c}{Uncensored} & \multicolumn{2}{c}{Interval Length}\\
        \cline{2-9}
         & Mean & Std.  & Mean & Std.  & Mean & Std.  & Mean & Std.\\
         \hline\hline 
         Cox Reg. & 0.996 & 0.003 & / & / & / & / & 319.84 & 2.78\\
         CoxPH & 0.995 & 0.003 & 0.994 &  0.005 & 0.995 & 0.005 & 340.20 & 6.85\\
        CoxCC & 0.996 & 0.004 & 0.994  &  0.005 & 0.998 & 0.004 & 344.26 & 6.93\\
        CoxPH+WCCI & 0.977 & 0.011 & 0.948 & 0.021 & 0.985 & 0.009 & 334.14 & 5.33 \\
        CoxPH+T-SCI & 0.986 & 0.009 & 0.970 & 0.016 & 0.989 & 0.008& 340.67 & 2.91\\
        CoxCC+WCCI & 0.973 & 0.014 & 0.942 & 0.027 & 0.980 & 0.012 & 334.28 & 5.36 \\ 
        CoxCC+T-SCI & 0.986 & 0.008 & 0.971 & 0.015 & 0.990 & 0.007 & 340.80 & 2.98\\
        CoxPH+WCCI(unweigted) & 0.946 & 0.031 & 0.910 & 0.055 & 0.972 & 0.021 & 254.56 & 8.38\\
        CoxPH+T-SCI(unweighted) & 0.958 & 0.063 & 0.932 & 0.063 & 0.977 & 0.021 & 261.18 & 9.26\\
        CoxCC+WCCI(unweigted) & 0.946 & 0.031 & 0.904 & 0.053 & 0.968 & 0.019 & 254.35 & 8.27\\
        CoxCC+T-SCI(unweighted) & 0.958 & 0.063 & 0.926 & 0.061 & 0.975 & 0.022 & 261.17 & 8.87\\
        Kernel & 0.981 & 0.025 & 0.997 & 0.010 & 0.971 & 0.038 & 337.66 & 20.39\\
        \hline 
    \end{tabular}
    \caption{metabric}
    \label{tab:m_res}
\end{table*}


